Automated Recurrence Analysis for Almost-Linear Expected-Runtime Bounds

We consider the problem of developing automated techniques for solving recurrence relations to aid the expected-runtime analysis of programs. Several classical textbook algorithms have quite efficient expected-runtime complexity, whereas the corresponding worst-case bounds are either inefficient (e.g., QUICK-SORT), or completely ineffective (e.g., COUPON-COLLECTOR). Since the main focus of expected-runtime analysis is to obtain efficient bounds, we consider bounds that are either logarithmic, linear, or almost-linear ($\mathcal{O}(\log n)$, $\mathcal{O}(n)$, $\mathcal{O}(n\cdot\log n)$, respectively, where n represents the input size). Our main contribution is an efficient (simple linear-time algorithm) sound approach for deriving such expected-runtime bounds for the analysis of recurrence relations induced by randomized algorithms. Our approach can infer the asymptotically optimal expected-runtime bounds for recurrences of classical randomized algorithms, including RANDOMIZED-SEARCH, QUICK-SORT, QUICK-SELECT, COUPONCOLLECTOR, where the worst-case bounds are either inefficient (such as linear as compared to logarithmic of expected-runtime, or quadratic as compared to linear or almost-linear of expected-runtime), or ineffective. We have implemented our approach, and the experimental results show that we obtain the bounds efficiently for the recurrences of various classical algorithms.

==> guess_and_check.tex <==
\section{Guess-and-Check Functions}\label{sect:mfunc}

We follow the standard guess-and-check technique to solve simple recurrence relations. 
Below we first fix a univariate recurrence relation $G$ taking the form (\ref{eq:unirecurrel}).

\smallskip
\begin{definition}[Univariate Guess-and-Check Functions]\label{def:uniguess}
Let $G$ be a univariate recurrence relation taking the form (\ref{eq:unirecurrel}). 
A function $h:\Nset\rightarrow\Rset$ is a \emph{guess-and-check} function for $G$ if there exists a natural number $N\in\Nset$ such that  
\begin{compactitem}
\item {\em (Base Condition)} $T_G(n)\le h(n)$ for all $1\le n\le N$, and
\item {\em (Inductive Argument)} $\Sub(\mathfrak{e},h) (n)\le h(n)$ for all $n> N$.  
\end{compactitem}
\end{definition}

By an easy induction on $n$ (starting from the $N$ specified in Definition~\ref{def:uniguess})
we obtain the following result. 

\medskip
\begin{theorem}[Guess-and-Check, Univariate Case]\label{thm:uniguess}
If a function $h:\Nset\rightarrow\Rset$ is a \emph{guess-and-check} function for a univariate recurrence relation $G$ taking the form (\ref{eq:unirecurrel}), then $T_G(n)\le h(n)$ for all $n\in\Nset$. 
\end{theorem} 
%%\begin{proof} \end{proof}

We do not present explicitly present the definition for guess-and-check functions in the bivariate case, 
since we will present a reduction of the analysis of separable bivariate recurrence relations to that 
of the univariate ones (cf. Section~\ref{sect:bisynth}). 

\begin{comment}
\begin{definition}[Bivariate Guess-and-Check Functions]\label{def:biguess}
Let $G$ be a bivariate recurrence relation taking the form (\ref{eq:birecurrel}).
A function $h:\Nset\times\Nset\rightarrow\Rset$ is a \emph{guess-and-check} function for $G$ if there exists a natural number $N\in\Nset$ such that
\begin{compactitem}
\item {\em (Base Condition)} $T_G(n,m)\le h(n,m)$ for all $n\in\Nset$ and $1\le m\le N$, and
\item {\em (Inductive Argument)} $\Sub(\mathfrak{e}, h)(n,m)\le h(n,m)$ for all $n\in\Nset$ and $m> N$.  
\end{compactitem}
\end{definition}

\smallskip
\begin{theorem}[Guess-and-Check, Bivariate Case] 
If a function $h:\Nset\times\Nset\rightarrow\Rset$ is a \emph{guess-and-check} function for a bivariate recurrence relation $G$ taking the form (\ref{eq:birecurrel}),
then $T_G(n,m)\le h(n,m)$ for all $n,m\in\Nset$. 
\end{theorem} 
\begin{proof}
By an easy induction on $m$ (starting from the $N$ specified in Definition~\ref{def:biguess}).
\end{proof}
\end{comment}




